On the pre- and post-positional semi-random graph processes

We study the semi-random graph process, and a variant process recently suggested by Nick Wormald. We show that these two processes are asymptotically equally fast in constructing a semi-random graph $G$ that has property ${\mathcal P}$, for the following examples of ${\mathcal P}$: - ${\mathcal P}$ is the set of graphs containing a $d$-degenerate subgraph, where $d\ge 1$ is fixed; - ${\mathcal P}$ is the set of $k$-connected graphs, where $k\ge 1$ is fixed. In particular, our result of the $k$-connectedness above settles the open case $k=2$ of the original semi-random graph process. We also prove that there exist properties ${\mathcal P}$ where the two semi-random graph processes do not construct a graph in ${\mathcal P}$ asymptotically equally fast. We further propose some conjectures on ${\mathcal P}$ for which the two processes perform differently.

==> Main_sections/k-connectednesswithcomments.tex <==
\section{$k$-Connectivity}
In their seminal paper, Ben-Eliezer et~al.~\cite{Ben-Eliezer2020Semi-randomProcess} provide tight asymptotic bounds for the \jt{minimum} number of rounds needed \jt{for a semi-random graph process} to \jt{produce an a.a.s.}\ $k$-vertex connected \jt{graph}, for all $k \geq 3$. Their proof for the upper bound is based on a slightly modified variant of the $k$-min process tailored for multigraphs and builds on a proof by Kang et~al.~\cite{Kang2006TheProcess}. The proof shows that the graph resulting from the modified $k$-min process is a.a.s. $k$-connected for all $k \geq 3$. This proof cannot be directly extended to $k < 3$, as Kang et~al.~\cite{Kang2006TheProcess} showed that the graph resulting from the $k$-min process is only a.a.s. connected for $k \geq 3$.

We moreover note that the case where $k = 1$, i.e. being connected, is trivial. Namely, we observe that one can build a tree containing $m \leq n -1$ edges in exactly $m$ rounds. If the first vertex chosen u.a.r. in a round is contained in the tree constructed thus far, we pick a vertex not contained in the tree, and vice versa. Hence, we can build a spanning tree in $n-1$ rounds. We moreover note that this is optimal, as spanning trees are edge-minimal 1-connected. \jc{Give a brief comment here about the pre-positional version (for $k=1$ only), and say it is going to be discussed ???}

    Therefore, this section will focus on proving tight asymptotic bounds for the final open case, $k = 2$. The best bound previously known, as observed by Ben-Eliezer et~al.~\cite{Ben-Eliezer2020Semi-randomProcess}, is the tight upper bound for $k = 3$. That is, $\tau_{\mathcal{C}_2} \leq \tau_{\mathcal{C}_3}$. They also gave a lower bound, based on the $2$-min process. The $2$-min process aims to ensure that each vertex has degree at least two as fast as possible, a prerequisite for $2$-connectedness. \jt{Using a known result by Wormald on the min-degree process,} they showed that \jt{2-min} process a.a.s.\ takes $(\ln 2 + \ln(\ln 2+1)) + o(1))n$ rounds to complete. Hence, \jt{$\tau_{\mathcal{C}_2} = \ln 2 + \ln(\ln 2+1)$.} \jc{was $\tau_{\mathcal{C}_2} \geq (\ln(2) + \ln(\ln(2)+1)) + o(1))n$. }

In this section we show a novel upper bound, \jt{which asymptotically matches the known lower bound.}

\begin{theorem}
    \label{thm:2-connectedness}
\jt{$\tau_{\mathcal{C}_2} = \ln 2 + \ln(\ln 2+1)$.}
    \jc{was:  
    $\tau_{\mathcal{C}_2} = (\ln(2) + \ln(\ln(2)+1)) + o(1))n$. }
\end{theorem}
\jt{In other words, the minimum number of rounds required for a semi-random process to build a $2$-connected graph on $[n]$ is asymptotic to $(\ln 2 + \ln(\ln 2+1))n$.}

Additionally, we consider property $\mathcal{C}_k$ in the pre-positional process. We show that all the proofs for the post-positional process extend to the pre-positional process, resulting in the following theorem.

\begin{theorem}
    \label{thm:equality_models_k-connectedness}
    $\tau_{\mathcal{C}_k}' = \tau_{\mathcal{C}_k}$ for all $k \geq 1$.
\end{theorem}

\subsection{Overview}
For the upper bound, our approach differs significantly from the strategy used by Ben-Eliezer et al.~\cite{Ben-Eliezer2020Semi-randomProcess} to prove \jt{the} tight upper bounds for \jt{the} $k$-connectedness for $k \geq 3$. Namely, while their approach is predominantly probabilistic, we use a more structural approach. Our strategy is based on analyzing the structure of the maximal 2-connected components of the graph resulting from the $2$-min process.

In the first phase, we use the $2$-min process to obtain a graph in which each vertex has degree at least $2$. We show that a.a.s. most of the vertices in this graph will be contained in relatively large $2$-connected subgraphs. This moreover allows us to conclude that the graph contains $o(n)$ maximal $2$-connected subgraphs. 

In the second phase, the aim is to ensure that the graph becomes connected. We bound the number of \jc{deleted: connected} components by the number of maximal $2$-connected subgraphs, \jt{recalling that we have shown that the graph obtained after the first phase has $o(n)$ maximal 2-connected subgraphs.} \jc{ showing that the graph contains few connected components.} As such, by adding edges between connected components, we can quickly ensure the graph becomes connected.

In the third phase, we then want to make the graph $2$-edge-connected. We achieve this by considering a tree structure on the maximal $2$-connected subgraphs, and showing that by balancing this tree, we can efficiently eliminate cut-edges.

In the fourth phase, we then add additional edges between the large maximal $2$-connected subgraphs to ensure that the majority of the graph is $2$-connected.

In the fifth and final phase, we then also absorb all the small components that were disregarded in the previous phase. Due to the small number of such vertices, we take a brute force approach.

We show that the second, third, fourth, and fifth phases all take $o(n)$ steps a.a.s. Therefore, the first phase, \jt{which is} the $2$-min process, dominates the \jt{total} number of rounds \jt{in the process of building a 2-connected graph on $[n]$}. 

In Section~\ref{subsection:supporting_structural_results}, we first introduce the purely structural definitions and results we will use. Section~\ref{subsection:proof_upper_bound_k-connectedness} then builds upon these structural results to analyze \jt{the random process given by} our strategy.

\subsection{Supporting structural results}
\label{subsection:supporting_structural_results}
In this section we restate the conventional definitions of blocks and block graphs (see for instance~\cite{Konig1936TheorieStreckenkomplexe}).

\begin{definition}[Block]
	\label{def:block}
	Let $B \subseteq V(G)$ be a maximal set of vertices such that for any two vertices $x, y \in B$ with $xy \not \in E(G)$, in order to separate vertex $x$ from vertex $y$, it is necessary to remove at least $2$ vertices from $G$. Then $B$ is called a block.
\end{definition}

Note that by this definition, each block in a graph either induces a maximal $2$-connected subgraph, or an edge. Based on this definition, we can then decompose a graph $G$ into such blocks.

\begin{definition}[Block decomposition]
	\label{def:block_decomposition}
	Let $\mathcal{B}(G) \subseteq \mathcal{P}(V(G))$ denote the set of all blocks of graph $G$. Then $\mathcal{B}(G)$ is called the block decomposition of graph $G$.
\end{definition}
We observe that by the definition of blocks, for each edge $uv \in E(G)$ in a graph $G$ there exists a \jt{unique} block $B \in \mathcal{B}(G)$ such that $u,v \in B$. \jt{Note also that in this definition, $\mathcal{B}(G)$ is usually not a partition of $V(G)$. However, each pair of blocks has intersection size at most one, as given in the following proposition.}



\begin{proposition}{\cite[Theorem~XIV.7]{Konig1936TheorieStreckenkomplexe}}
	\label{prop:max_intersect_block}
	Let $G$ be a graph. Then, for each pair of blocks $B_1, B_2 \in \mathcal{B}(G)$, it holds that $|B_1 \cap B_2| \leq 1$.
\end{proposition}
\begin{comment}
\begin{proof}
    Suppose not. Then let $B_1, B_2 \in \mathcal{B}$ be blocks such that $|B_1 \cap B_2| \geq 2$. By the maximality of blocks $B_1$ and $B_2$, neither $B_1 \subset B_2$ nor $B_2 \subset B_1$. Hence, $|B_1|, |B_2| \geq 3$, and thus both blocks $B_1$ and $B_2$ induce $2$-connected subgraphs. Moreover, by the maximality of blocks $B_1$ and $B_2$, vertex set $B_1 \cup B_2$ does not induce a $2$-connected graph. Let $u_1, u_2 \in B_1 \cap B_2$. Additionally, let $v_1, v_2 \in B_1 \cup B_2$ be vertices such that deleting one vertex from graph $G$ separates vertices $v_1$ and $v_2$. 
    
    As blocks $B_1$ and $B_2$ induce $2$-connected subgraphs, $|B_1\cap \{v_1, v_2\}| = |B_2 \cap \{v_1, v_2\}| = 1$. Then, without loss of generality, assume that $v_1 \in B_1 \setminus B_2$, and $v_2 \in B_2 \setminus B_1$. Additionally, without loss of generality assume that deleting vertex $w \in B_1$ separates vertices $v_1$ and $v_2$. We note that as block $B_1$ is $2$-connected, $B_1 \setminus \{w\}$ induces a connected subgraph in graph $G$. Moreover, $B_1 \setminus \{w\}$ contains at least one of the vertices $u_1, u_2$. Without loss of generality, assume $u_1 \in B_1 \setminus \{w\}$. But then, as $B_2 \setminus \{w\}$ is connected, and $v_2 \neq w$, there exist $v_1-u_1$ and $u_1-v_2$ paths, and thus a $v_1-v_2$ paths in graph $G - w$, contradicting the definition of vertices $v_1$, $v_2$ and $w$. we thus conclude that the proposition holds.
\end{proof}
\end{comment}

\jc{Add discussions of the uniqueness of block decompositions.}

\begin{definition}[Block graph]
	\label{def:block_graph} 
	Let $G$ be a graph. Then let $G_{\mathcal{B}}$ be the graph defined by $V(G_{\mathcal{B}}) = \mathcal{B}(G)$ and $E(G_{\mathcal{B}}) = \{B_1B_2 \, : \, B_1 \cap B_2 \neq \emptyset\}$.  Then graph $G_{\mathcal{B}}$ is called the block graph of graph $G$.
\end{definition}
\begin{comment}
    Moreover, let $w : E(G_{\mathcal{B}}) \to \mathbb{R}^+$ be a function assigning weights to each edge in graph $G_{\mathcal{B}}$, defined by $w(B_1B_2) = \sum_{v \in B_1 \cap B_2} 2/\left(f(v)\cdot(f(v)-1)\right)$ for each edge $B_1B_2 \in E(G_{\mathcal{B}})$ where $f(v)$ is the number of blocks containing vertex $v5$, i.e. $f(v) = |\{B \in \mathcal{B}\, : \, v \in B\}|$.
\end{comment}

\begin{comment}
\begin{proposition}
	\label{prop:mincut_subgraph}
	Let $H_{\mathcal{B}}$ be a non-trivial induced subgraph of reduced $k$-block graph $G_{\mathcal{B}}$ of graph $G$. Then subgraph $H_{\mathcal{B}}$ admits a cut of value at most $k-1$.
\end{proposition}
\begin{proof}
	Let $H$ be the subgraph of graph $G$ induced by the vertex set $\bigcup_{v_B \in V(H_{\mathcal{B}})} B$. Additionally, let $\mathcal{B}' = \{B \in \mathcal{B} \, : \, v_B \in V(H_{\mathcal{B}})$. We first consider the case that subgraph $H_{\mathcal{B}}$ contains a vertex $v_B$ such that $|B| \leq k-1$. We then consider the set $F \subseteq E(H_{\mathcal{B}})$ consisting of all the edges incident to vertex $v_B$. As subgraph $H_{\mathcal{B}}$ is non-trivial, and as vertex $v_B$ is an isolated vertex in $H_{\mathcal{B}}\setminus F$, $F$ is a cut. We then bound the value of this cut:
	\begin{align*}
	\sum_{v_{B}v_{B'} \in F} w(v_Bv_{B'}) &= \sum_{v_{B'} \in N(v_B)}w(v_Bv_{B'})\\
	&= \sum_{v_{B'} \in N(v_B)} \sum_{v \in B \cap B'} \frac{2}{f(v)\cdot (f(v) -1)}\\
	&= \sum_{v \in B} \sum_{v_{B'} \in N(v_B) \, : \, v \in B'}\frac{2}{f(v)\cdot (f(v)-1)}\\
	&\leq \sum_{v\in B} |\{B' \in \mathcal{B} \, : \, v \in B'\} \setminus \{B\}| \cdot \frac{2}{f(v)\cdot (f(v) -1)}\\
	&= \sum_{v\in B} (f(v)-1) \cdot \frac{2}{f(v)\cdot (f(v) -1)}\\
	&\leq \sum_{v\in B} 1\\
	&= |B|\\
	&\leq k -1
	\end{align*}
	Thus, set $F$ is a cut of value at most $k-1$ of subgraph $H_{\mathcal{B}}$, as desired.
	
	Hence we may assume that $|B| \geq k$ for all $B \in \mathcal{B}'$. We then note that as $H_{\mathcal{B}}$ is non-trivial, $|V(H)| \geq k + 1$. Moreover, by the maximality of the $k$-blocks in $\mathcal{B}$, subgraph $H$ is not $k$-connected. Let $v_1,v_2 \in V(H)$ be a pair of vertices in subgraph $H$ such that vertices $v_1$ and $v_2$ can be separated by removing at most $k-1$ vertices. Let $S \subseteq V(H) \setminus \{v_1,v_2\}$ be a minimal set of vertices such that vertices $v_1$ and $v_2$ are not contained in the same connected component of $H - S$. Thus, $|S| \leq k-1$.
	
	Because $|B| \geq k$ for all $B \in \mathcal{B}'$, by the definition of a $k$-block, each $k$-block $B \in \mathcal{B}'$ induces a $k$-connected subgraph in graph $G$. Hence, vertices $v_1$ and $v_2$ are contained in distinct $k$-blocks $B_1$ and $B_2$ respectively, such that $v_1 \not \in B_2$ and $v_2 \not \in B_1$. Moreover, we note that as at least $k$ vertices are required to disconnect vertices within a $k$-block, by the minimality of $S$, set $S$ only contains boundary vertices. Hence, for all vertices $v \in S$, it holds that $f(v) \geq 2$.
	
	Let $C_1$ and $C_2$ be the connected components of graph $H - S$ containing vertices $v_1$ and $v_2$ respectively. Because no $k$-block $B \in \mathcal{B}'$ is disconnected into multiple connected components by removing the vertices of set $S$, for each $k$-block $B \in \mathcal{B}'$ it holds that $B \cap V(C_1) = \emptyset$ or $B \cap V(C_2) = \emptyset$. Let $\mathcal{B}_1 \subseteq \mathcal{B}'$ be the set of $k$-blocks $B \in \mathcal{B}'$ such that $B \cap V(C_1) \neq \emptyset$, and let $\mathcal{B}_2 \subseteq \mathcal{B}'$ consist of the remaining $k$-blocks in set $\mathcal{B}'$, that is, $\mathcal{B}_2 = \mathcal{B}' \setminus \mathcal{B}_1$.
	
	Then, let $F \subseteq E(H_{\mathcal{B}})$ be the set of edges in subgraph $H_{\mathcal{B}}$ with exactly one endpoint in the set $\{v_{B'} \, : \, B' \in \mathcal{B}_1\}$ and exactly one endpoint in the set $\{v_{B'} \, : \, B' \in \mathcal{B}_2$. Thus, set $F$ is a cut of subgraph $H_{\mathcal{B}}$. We then bound the value of cut $F$:
	\begin{align*}
	\sum_{B_1 \in \mathcal{B}_1}\sum_{B_2 \in \mathcal{B}_2} w(v_{B_1}v_{B_2}) &= \sum_{B_1 \in \mathcal{B}_1}\sum_{B_2 \in \mathcal{B}_2} \sum_{v \in B_1 \cap B_2} \frac{2}{f(v) \cdot (f(v) - 1)}\\
	&=\sum_{v \in S} \sum_{B_1 \in \mathcal{B}_1 \, : \, v \in B_1} \sum_{B_2 \in \mathcal{B}_2 \, : \, v \in B_2} \frac{2}{f(v) \cdot (f(v) -1 )}\\
	&= \sum_{v \in S} |\{B_1 \in \mathcal{B}_1 \, : \, v \in B_1\}| \cdot |\{B_2 \in \mathcal{B}_2 \, : \, v \in B_2\}| \cdot \frac{2}{f(v) \cdot (f(v) - 1)}\\
	&\leq \sum_{v \in S} \frac{f(v)}{2} \cdot \frac{f(v)}{2} \cdot \frac{2}{f(v)(f(v) - 1)}\\
	&= \sum_{v \in S} \frac{f(v)}{2f(v) - 2}\\
	&\leq \sum_{v\in S} 1\\
	&= |S|\\
	&\leq k-1
	\end{align*}
	Thus, set $F$ is a cut of value at most $k-1$ of subgraph $H_{\mathcal{B}}$, as desired.
\end{proof}
\end{comment}


For a graph $G$ to be $2$-connected, it must hold that $\mathcal{B}(G) = \{V(G)\}$. We aim to use the blocks and their relative structure in a graph to identify \jt{moves in a semi-random process} \jc{was: augmentations} which join multiple blocks together \jt{into} a single larger block. \jt{If a semi-random edge $u_tv_t$ joins two blocks then we call the addition of such an edge an {\em augmentation}.} A natural augmentation to consider is \jt{to join two blocks $B_i$ and $B_j$, where there is a (hopefully long) path between $B_i$ and $B_j$ in $G_{{\cal B}}$. This augmentation will immediately join all blocks along the path to a single block.} \jc{was: forming a cycle of blocks.} To that purpose, we want to consider a tree structure on the blocks. \jc{deleted, because it is ambiguous: such that cycles are easily constructed on the blocks.}

The traditional such structure, called the block-cut tree of a graph, was originally introduced independently by Gallai~\cite{Gallai1964ElementareGraphen}, and Harary and Prins~\cite{Harary1966TheGraph}.

\begin{definition}[Block-cut tree]
    \label{def:block-cut_tree}
    Let $G$ be a graph, and let $S$ be the set of cut vertices of graph $G$. Then, the graph $T$, given by $V(T) = \mathcal{B}(G) \cup S$ and $E(T) = \{vB \, | \, v \in S, B \in \mathcal{B}(G), v \in B\}$, is a tree and called the block-cut tree of graph $G$. 
\end{definition}



\begin{comment}
\begin{lemma}
	\label{lem:k-block_structure}
	Let $S \subseteq \mathcal{P}(V(G))$ be a set of $k$-blocks in graph $G$ where $|B| > k$ for all $k$-blocks $B \in S$. Then, the number of vertices $v \in V(G)$ contained in multiple $k$-blocks in set $S$ is at most $(|S|-1) \cdot (k-1)$.
\end{lemma}
\begin{proof}
	Suppose not. Then let $S \subseteq \mathcal{P}(V(G))$ be a minimal counter example. If $|S|=1$, the lemma trivially holds. Hence we may assume $|S| \geq 2$. Let $G_{\mathcal{B}}$ be the $k$-block graph of graph $G$, and let $G_S$ be the subgraph of $G_{\mathcal{B}}$ induced by the vertex set $\{v_B \, : \, B \in S\}$. 
	\textcolor{red}{TODO finish proof, be careful about restricting reduced $k$-block graph to $S$}
\end{proof}
\end{comment}

We consider a structure similar to the block-cut tree, based on the block graph. Instead of including the cut-vertices in the tree, we take a spanning tree on the block graph. This ensures that we only have to work with blocks, while still providing the desired tree structure. To that aim, we introduce the following definition.

\begin{definition}[Reduced block tree]
    \label{def:reduced_block_tree}
    Let $G_{\mathcal{B}}$ be the block graph of a connected graph $G$. Then, a spanning tree $T_{\mathcal{B}}$ of graph $G_{\mathcal{B}}$ is called a reduced block tree of graph $G$.
\end{definition}

\jc{For your thesis, it is better to insert a figure with an example here: draw a graph, then draw $G_{{\cal B}}$, and then draw the block-cut tree, then draw the reduced block tree.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Blocktrees.png}
    \caption{Illustration of the different structural representations of the block decomposition $\mathcal{B}$ of graph $G$.}
    \label{fig:blocktrees}
\end{figure}

\jc{Personally I still feel that the block-cut tree is more natural to be used for our analysis.}

\jc{slight restructuring below.}

A reduced block tree can equivalently be constructed recursively. Let $v \in V(G)$ be a cut-vertex in a connected graph $G$, and let $G_1$ and $G_2$ be the induced subgraphs of graph $G$ such that $V(G_1) \cup V(G_2) = V(G)$, $E(G_1) \cup E(G_2) = E(G)$, and $V(G_1) \cap V(G_2) = \{v\}$. We note that as vertex $v$ is a cut-vertex, each block $B \in \mathcal{B}(G)$ is contained in either graph $G_1$ or graph $G_2$. Therefore, $\mathcal{B}(G_1) \cup \mathcal{B}(G_2) = \mathcal{B}(G)$.  Let $T_{\mathcal{B}_1}$ and $T_{\mathcal{B}_2}$ be reduced block trees for graphs $G_1$ and $G_2$ respectively. Then, we can construct a reduced block tree for graph $G$ \jt{given a} block decomposition $\mathcal{B}$ by joining trees $T_{\mathcal{B}_1}$ and $T_{\mathcal{B}_2}$ with a single edge from \jt{a} vertex in $T_{\mathcal{B}_1}$ representing a block containing vertex $v$ to a vertex in $T_{\mathcal{B}_2}$ also representing a block containing vertex $v$. We observe that by \jt{Definition~\ref{def:reduced_block_tree}}, the reduced block tree of a graph is generally not unique. \jt{This happens when a vertex is contained in more than two blocks.}

\begin{proposition}
    \label{prop:reduced_block_tree_leaves}
    Let $T_{\mathcal{B}}$ be a reduced block tree of a connected graph $G$. If each vertex in \jc{deleted: graph} $G$ has degree at least $2$, \jt{then} each leaf in \jc{deleted: tree} $T_{\mathcal{B}}$ corresponds to a $2$-connected block in graph $G$ of at least $3$ vertices.
\end{proposition}
\begin{proof}
    Suppose not. Then let \jc{deleted: vertex} $B \in V(T_{\mathcal{B}})$ be a leaf of \jc{deleted: tree} $T_{\mathcal{B}}$ such that the corresponding block $B = \{u,v\}$ consists of two vertices, inducing an edge in \jc{deleted: graph} $G$. 
    Because each vertex in \jc{deleted: graph} $G$ has degree at least two, \jc{deleted: vertex $u$} has a neighbor $u' \in V(G) \setminus \{v\}$ in graph $G$, and similarly vertex $v$ has a neighbor $v' \in V(G) \setminus \{u\}$ in graph $G$. We note that $u' \neq v'$, as otherwise $\{u,v,u'\}$ would induce a cycle and thus a $2$-connected subgraph in $G$, contradicting the maximality of block $B$. By an analogous argument, there does not exist a path between vertices $u$ and $v$ in graph $G - uv$. However, as by the definition of a block composition there exist blocks $B_1, B_2 \in \mathcal{B}(G)$ containing edges $uu'$ and $vv'$ respectively. \jc{deleted: and as such vertices in tree $T_{\mathcal{B}}$ representing said blocks.} Moreover, \jc{deleted: tree} $T_{\mathcal{B}} - B$ is a valid reduced block tree for \jc{deleted: graph} $G - uv$. But then, as a reduced block tree is by definition a spanning tree of the blocks, there exists a path between vertices $B_1$ and $B_2$ in tree $T_{\mathcal{B}} - B$, and hence a path between vertices $u$ and $v$ in graph $G - uv$, a contradiction. Hence, we conclude that a leaf of \jc{deleted: tree} $T_{\mathcal{B}}$ cannot represent a block of two vertices, as desired.
\end{proof}

\begin{proposition}
    \label{prop:reduced_block_tree_subtrees}
    Let $T_{\mathcal{B}}$ be a reduced block tree of a connected graph $G$. For $v \in V(G)$, the set $\{B \in V(T_{\mathcal{B}}) \, : \, v \in B\}$ induces a (connected) subtree \jt{of} \jc{deleted: tree} $T_{\mathcal{B}}$.
\end{proposition}
\begin{proof}
    Suppose not. Let $S \subseteq V(T_{\mathcal{B}})$ be the set of all blocks $B \in V(T_{\mathcal{B}})$ such that $v \in B$. Then the set $S$ induces a \jt{disconnected} \jc{was: non-connected} subgraph in tree $T_{\mathcal{B}}$. Let $C_1$ and $C_2$ be two \jc{deleted: connected} components of this induced subgraph $T_{\mathcal{B}}[S]$. Moreover, let $P$ be a shortest path between sets $V(C_1)$ and $V(C_2)$ in \jc{deleted: tree} $T_{\mathcal{B}}$, and let blocks $B_1, B_2 \in S$ be the endpoints of this path $P$ such that $B_1 \in V(C_1)$ and $B_2 \in V(C_2)$. We note that $P$ has length at least 2. Then, as $P$ is a shortest such path, none of the internal vertices of \jc{deleted: path} $P$ are contained in $S$. Hence, the corresponding blocks do not contain vertex $v$. Let $G_P$ be \jt{the subgraph of $T_{\mathcal{B}}$ induced} by the internal vertices of path $P$. Additionally, let $S_P \subseteq V(G)$ be the set of all vertices of graph $G$ contained in at least one of the blocks \jc{deleted: represented in subgraph} \jt{in} $G_P$.
    
    We observe that by the definition of path $P$, subgraph $G_P$ contains blocks adjacent to blocks $B_1$ and $B_2$ respectively in tree $T_{\mathcal{B}}$. Therefore, $B_1 \cap S_P, B_2 \cap S_P \neq \emptyset$. Moreover, by Proposition~\ref{prop:max_intersect_block} we find that $B_1 \cap B_2 = \{v\}$. Therefore, as $v \not \in S_P$, there exist vertices $v_1 \in B_1 \cap S_P$ and $v_2 \in B_2 \cap S_P$. Then, because blocks $B_1$ and $B_2$ are by definition connected, there exists a  \jc{was: $v-v_1$} \jt{$v,v_1$-}path $P_1$ in block $B_1$ and a $v,v_2$-path $P_2$ in block $B_2$. Similarly, set $S_P$ induces a connected subgraph \jc{deleted: in graph} \jt{of} $G$, and thus contains a $v_1,v_2$-path $P'$. We note that the union of the paths $P_1$, $P_2$ and $P'$ gives a subgraph of \jc{deleted: graph} $G$ containing a cycle $C$ containing vertex $v$. We note that cycle $C$ is 2-connected and hence is contained in a block $B_C$. Moreover, as this cycle contains at least 2 vertices of block $B_1$, by Proposition~\ref{prop:max_intersect_block}, we find that $B_1 = B_C$. Analogously, it follows that $B_2 = B_C$. However, this implies that $B_1 = B_2$, contradicting these blocks being in different connected components $C_1$ and $C_2$. By this contradiction, we conclude that the proposition holds.
\end{proof}

\begin{proposition}
    \label{prop:reduced_block_tree_balanced}
    Let $G$ be a connected graph such that $|B| < n/4$ for all blocks $B \in \mathcal{B}(G)$, and let $T_{\mathcal{B}}$ be a corresponding reduced block tree. Then there exists a vertex ${B^*} \in V(T_{\mathcal{B}})$ and a coloring $\phi : V(T_{\mathcal{B}}) \setminus \{B^*\} \to \{\text{red$,$ blue}\}$ such that all \jc{deleted: the  connected} components of \jc{deleted:forest} $T_{\mathcal{B}} - {B^*}$ are monochromatic and that for $S_{\text{red}} = \{v \in B \setminus B^* \, : \, B \in \mathcal{B}, \phi(B) = \text{red}\}$ and $S_{\text{blue}} = \{v \in B \setminus B^* \, : \, B \in \mathcal{B}, \phi(B) = \text{blue}\}$ it holds that $|S_{\text{blue}}| \leq |S_{\text{red}}| \leq 3|S_{\text{blue}}|$.
\end{proposition}
\begin{proof}
    Firstly, we note by Proposition~\ref{prop:reduced_block_tree_subtrees} that $S_{\text{red}} \cap S_{\text{blue}} = \emptyset$ and hence $V(G)$ is partitioned by the sets $B^*$, $S_{\text{red}}$, and $S_{\text{blue}}$. Therefore, $|B^*| + |S_{\text{red}}| + |S_{\text{blue}}| = n$.
    
    Assume that the proposition does not hold. Then, let ${B^*} \in V(T_{\mathcal{B}})$ and $\phi : V(T_{\mathcal{B}}) \to \{\text{red$,$blue}\}$ be a vertex and a coloring respectively such that all \jc{deleted:the connected} components of \jc{deleted:forest} $T_{\mathcal{B}} - {B^*}$ are monochromatic, $|S_{\text{red}}| \geq |S_{\text{blue}}|$, and $|S_{\text{red}}|$ minimized. We note that as it concerns a counterexample, we must have $|S_{\text{red}}| > 3|S_{\text{blue}}|$. 
    
    We observe that as $|B^*| < n/4$, \jc{deleted:forest} $T_{\mathcal{B}} - {B^*}$ is non-empty. Therefore, due to $|S_{\text{red}}| \geq |S_{\text{blue}}|$, \jc{deleted:forest} $T_{\mathcal{B}} - {B^*}$ contains at least one red \jc{deleted:connected} component. Suppose that \jc{deleted:forest} $T_{\mathcal{B}} - {B^*}$ contains exactly one red \jc{deleted:connected} component. Then, because \jc{deleted:graph} $T_{\mathcal{B}}$ is a tree, vertex ${B^*}$ has exactly one red neighbor ${B'} \in V(T_{\mathcal{B}})$ in tree $T_{\mathcal{B}}$. Then consider using vertex ${B'}$ instead of vertex ${B^*}$, uncoloring \jc{deleted:vertex} ${B'}$ and coloring \jc{deleted:vertex} ${B^*}$ blue. \jt{Let $\phi'$ denote the resulting new colouring,} \jc{For the paper, I would prefer to change all American spelling to British or Canadian, i.e. color to colour etc.} \jt{and} let $S_{\text{red}}'$ and $S_{\text{blue}}'$ be the sets of vertices in \jc{deleted:graph} $G$ corresponding to \jt{$\phi'$}. \jc{deleted: defined analogously to $S_{\text{red}}$ and $S_{\text{blue}}$.}  We note that as blocks $B^*$ and $B'$ contain less than $n/4$ vertices, it holds that $|S_{\text{red}}'| > |S_{\text{red}}| - n/4$ and $|S_{\text{blue}}'| < |S_{\text{blue}}| + n/4$. Moreover, we note that by the maximality of blocks, $B^* \setminus B', B' \setminus B^* \neq \emptyset$, and hence $|S_{\text{red}}'| < |S_{\text{red}}|$ and $|S_{\text{blue}}'| > |S_{\text{blue}}|$. If $|S_{\text{red}}'| > |S_{\text{blue}}'|$, the new coloring $\phi'$ is more balanced, and thus contradicts the minimality of $|S_{\text{red}}|$. Therefore, it holds that $|S_{\text{red}}'| < |S_{\text{blue}}'|$. Because we assumed that $|S_{\text{red}}| > 3|S_{\text{blue}}|$, and as $|B^*| + |S_{\text{red}}| + |S_{\text{blue}}| = n$, it follows that $|S_{\text{blue}}| \leq n/4$. Thus, $|S_{\text{blue}}'| < |S_{\text{blue}}| + n/4 \leq n/2$. But then, as $|B'| + |S_{\text{red}}'| + |S_{\text{blue}}'| = n$, it follows that
    \begin{align*}
        |S_{\text{red}}'| &= n - |S_{\text{blue}}'| - |B'|\\
        & > n - \frac{n}{2} - \frac{n}{4}\\
        &= \frac{n}{4}.
    \end{align*}
    Then, inverting the colors red and blue results in a coloring satisfying all the conditions of the proposition, contradicting  $T_{\mathcal{B}}$ being a counterexample.

    Hence, we may assume that forest $T_{\mathcal{B}} - {B^*}$ contains at least 2 red  components. Then let $C_1, C_2, \ldots, C_{\ell}$ be the red components of $T_{\mathcal{B}} - {B^*}$, and let $S_1, S_2, \ldots , S_{\ell}$ be defined by $S_i = \{v \in B \setminus B^* \, : \, B \in C_i\}$ for $i \in [\ell]$. Then, by Proposition~\ref{prop:reduced_block_tree_subtrees}, the sets $S_1, S_2, \ldots , S_{\ell}$ partition set $S_{\text{red}}$.
    
    Suppose that there exists an index $i \in [\ell]$ such that $|S_i| > |S_{\text{blue}}|$. Then, recoloring all blue components red, and recoloring component $C_i$ blue leads to sets $S_{\text{red}}'$ and $S_{\text{blue}}'$ such that, as $\ell \geq 2$, $\min(|S_{\text{red}}'|, |S_{\text{blue}}'|) > \min(|S_{\text{red}}|, |S_{\text{blue}}|)$. Thus, as $|S_{\text{red}}'| + |S_{\text{blue}}'| = |S_{\text{red}}| + |S_{\text{blue}}|$, \jt{by possibly inverting the colors, we find a new colouring (with the same choice of $B^*$) where $S_{\text{red}}$ is smaller, contradicting with our choice of $\phi$.} \jc{slight rewording of: we find a more minimal counterexample, possibly requiring inverting the colors.} Hence, we may assume that $|S_i| \leq |S_{\text{blue}}|$ for all $i \in [\ell]$. Then, as $|S_{\text{red}}| = \sum_{i=1}^{\ell} |S_i|$, we find that $|S_{\text{red}}| \leq \ell |S_{\text{blue}}|$. Therefore, as $|S_{\text{red}}| > 3|S_{\text{blue}}|$, it holds that $\ell > 3$.
    
    Similarly, suppose that there exists an index $i \in [\ell]$ such that $|S_i| < (|S_{\text{red}}| - |S_{\text{blue}}|) /2$. Then clearly recoloring component $C_i$ blue contradicts the minimality of $|S_{\text{red}}|$. Hence, we may assume that $|S_i| \geq (|S_{\text{red}}| - |S_{\text{blue}}|) /2$ for all $i \in [\ell]$. Then, as $|S_{\text{red}}| = \sum_{i=1}^{\ell} |S_i|$, we find that $|S_{\text{red}}| \geq \ell \cdot (|S_{\text{red}}| - |S_{\text{blue}}|) /2$. It then follows that, because $\ell > 3$, $|S_{\text{red}}| \leq \frac{\ell}{\ell - 2} |S_{\text{blue}}|$. But then, as $\frac{\ell}{\ell - 2} < 3$ for $\ell > 3$, we conclude that vertex ${B^*}$ and coloring $\phi$ do not form a counterexample.  \jc{deleted: contradicting their definition.} Thus, we conclude that the proposition holds.
\end{proof}

\subsection{\jt{Building $2$-connected semi-random graphs}}
\label{subsection:proof_upper_bound_k-connectedness}
In this section, we describe \jc{deleted: and analyze} our strategy \jt{for building a $2$-connected semi-random graph, and we analyse the random process produced by the strategy, and obtain the tight} upper bound of $\tau_{\mathcal{C}_2}$ \jt{as in Theroem~\ref{thm:2-connectedness}. Our strategy consists of five phases.} 

In the first phase, we use the $2$-min process, as previously described. The following proposition shows useful properties of the resulting graph.

\begin{proposition} 
    \label{prop:2-connectedness_small_blocks}
    Let $G$ be the semi-random graph resulting from the $2$-min process. Then, a.a.s., $G$ contains $o(n)$ vertices that are contained in $2$-connected induced subgraphs of order at most $\sqrt{\ln(n)}$ in graph $G$.
\end{proposition}
\begin{proof}
\jc{Reworded and polished at various places that I did not bother to mark.}
Let $X$ be the number of vertices contained in $2$-connected induced subgraphs of order at most $\sqrt{\ln n}$.
    We note that it suffices to show that $\ex{X}=o(n)$. Moreover, let $Y_\ell$ denote the number of $2$-connected induced subgraphs of order $\ell$ for $1 \leq \ell \leq \sqrt{\ln n}$. Thus, by linearity of expectation, $\mathbb{E}[X] \leq \sum_{\ell = 1}^{\sqrt{\ln n}} \ell \mathbb{E}[Y_\ell]$.
    
    For $1 \leq \ell \leq \sqrt{\ln(n)}$, let $Z_\ell$ denote the number of induced subgraphs of order $\ell$ with at least $\ell$ edges. Because each $2$-connected graph contains at least as many edges as the vertices, it follows immediately that $Y_\ell \leq Z_\ell$, and thus,  $\ex{X} \leq \sum_{\ell = 1}^{\sqrt{\ln(n)}} \ex{\ell Z_\ell}$. Hence it suffices to show that $\sum_{\ell = 1}^{\sqrt{\ln(n)}} \mathbb{E}[\ell Z_\ell] = o(n)$.


    
 \jc{was:    Then, we observe that $\mathbb{E}[Z_\ell]$ is equal to $\binom{n}{\ell}p_\ell$, where $p_\ell$ is the probability that a subgraph induced by $\ell$ vertices contains at least $\ell$ edges. Thus, $\sum_{\ell = 1}^{\ln(n)} \ell Z_\ell = \sum_{\ell = 1}^{\ln(n)}\ell \binom{n}{\ell}p_\ell$.}

 \jt{Let $1\le\ell\leq \sqrt{\ln n}$, and fix $S\subseteq [n]$ such that $|S|=\ell$. Let $p_S$ be the probability that $G[S]$ contains at least $\ell$ edges. Note that $\ex{Z_{\ell}}=\sum_{S\in \binom{[n]}{\ell}}p_S$. Next, we estimate $p_S$.}
    
    \jt{We first split the 2-min process into two phases. The first phase ends after the step where isolated vertices all disappear, and thus the second phase starts with a graph with minimum degree one. We further}   split each phase into subphases for analysis. Specifically, \jc{deleted: for the first phase, which ensures that each vertex has degree at least one,} we define subphases $\alpha_1, \alpha_2, \ldots$ such that $\alpha_i$ \jt{consists of the steps where} such that $\frac{n}{2^i} < |\{v \in V(G) \, | \, \deg(v) = 0\}| \leq \frac{n}{2^{i-1}}$ for $i = 1, 2, \ldots$.  We note that these subphases are well defined, as by the definition of the first phase of the $2$-min process, the number of isolated vertices is strictly decreasing \jt{in each step}. \jt{Then we} define subphases $\beta_1, \beta_2, \ldots$ of the second phase the 2-min process such that subphase \jt{$\beta_i$ consists of the steps where} $\frac{n}{2^i} < |\{v \in V(G) \, |  \, \deg(v) = 1\}| \leq \frac{n}{2^{i-1}}$ for $i = 1, 2, \ldots$. \jt{Note that some of the subphases might be empty, e.g.\ subphase $\beta_1$ is empty if the number of vertices with degree 1 at the beginning of phase 2 is already smaller than $n/2$.} 
    We observe that there are $\log_2(n)$  subphases of both phases of the $2$-min process.
    

    \jt{To bound $p_S$, we first choose a set $T$ of $\ell$ edges from $\binom{S}{2}$. There are $\binom{{\binom{\ell}{2}}}{\ell}\le \binom{\ell^2}{\ell}$ ways to do this. Then we set an ordering for edges in $T$. There are $\ell!$ ways to fix such an ordering. Fixing an ordering $e_1,\ldots, e_{\ell}$, we bound the probability that these edges are added to $G$ in this order.  The probability that a particular edge $xy\in T$ is added in a specified step in subphase $\alpha_i$ (and $\beta_i$) is at most $2\cdot\frac{1}{n}\cdot \frac{2^{i-1}}{n} = \frac{2^{i}}{n^2}$ (and same for $\beta_i$ respectively), since the first vertex of the edge is chosen uniformly at random, and the second vertex is chosen uniformly from the isolated vertices, and there are at most $n/2^{i-1}$ of them. The factor 2 accounts for whether $x$ or $y$ is the square of the edge (note that sometimes there can be only one option).  
    Let $\ell_{\alpha_i}$ and $\ell_{\beta_i}$ be the number of edges of $e_1,\ldots, e_{\ell}$ that are added in subphases $\alpha_i$ and $\beta_i$ respectively. Let ${\boldsymbol \ell_{\alpha}}=(\ell_{\alpha_i})_{i\ge 0}$ and ${\boldsymbol \ell_{\beta}}=(\ell_{\beta_i})_{i\ge 0}$.
    Note that the number of isolated vertices decreases by at least 1 in each step of the first phase of the $2$-min process. Thus the number of steps in subphase $\alpha_i$ is at most $\frac{n}{2^{i-1}}-\frac{n}{2^i} = \frac{n}{2^i}$. Thus, given ${\boldsymbol \ell_{\alpha}}$ and ${\boldsymbol \ell_{\beta}}$, there are at most $\prod_i \binom{n/2^i}{\ell_{\alpha_i}}\binom{n/2^i}{\ell_{\beta_i}}$ ways to specify steps in the 2-min process where edges in $T$ are added.
    Combining all, we have the following bound on $p_S$:
    }
    
%    We then note that as each round in the first phase of the $2$-min process decreases the number of isolated vertices by at least 1, the number of rounds in subphase $\alpha_i$ is at most $\frac{n}{2^{i-1}}-\frac{n}{2^i} = \frac{n}{2^i}$. Moreover, because the first vertex is chosen uniformly at random from all vertices in the graph, and as the second vertex is chosen uniformly at random from all isolated vertices, the probability that a specific edge is added in subphase $\alpha_i$ is at most $\frac{1}{n}\cdot \frac{2^{i-1}}{n} = \frac{2^{i-1}}{n^2}$, and analogously in subphase $\beta_i$. Then, if we let $\ell_{\alpha_i}$ and $\ell_{\beta_i}$ be the number of edges in a subgraph added in subphases $\alpha_i$ and $\beta_{i}$ respectively, we find that 

\[p_S \leq \binom{\ell^2}{\ell} \jt{\ell!}\sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}} } \left(\prod_{i = 1}^{\log_2(n)} \binom{n/2^i}{\ell_{\alpha_i}}\binom{n/2^i}{\ell_{\beta_i}} \left( \frac{2^{\jt{i}}}{n^2} \right)^{\ell_{\alpha_{i}}+\ell_{\beta_{i}}}  \right), \]
\jt{where the first summation above is over all choices where $\sum_{i=1}^{\log_2(n)} \left(\ell_{\alpha_i}+\ell_{\beta_i}\right)= \ell$.}


\jc{was:

\[p_S \leq \binom{\ell^2}{\ell} \sum_{\ell_{\alpha_i}, \ell_{\beta_i} \, : \, \sum_{i=1}^{\log_2(n)} \left(\ell_{\alpha_i}+\ell_{\beta_i}\right)= \ell} \left(\prod_{i = 1\, , \,\ell_{\alpha_i} \neq 0\, , \, \ell_{\beta_i} \neq 0}^{\log_2(n)} \left( \frac{n}{2^i \ell_{\alpha_i}}\cdot \frac{2^{i-1}}{n^2} \right)^{\ell_{\alpha_{i}}} \cdot \left( \frac{n}{2^i \ell_{\beta_i}}\cdot \frac{2^{i-1}}{n^2} \right)^{\ell_{\beta_{i}}} \right). \]

}

\jc{was:

    \begin{align*}
		p_s &\leq \binom{\ell^2}{\ell} \ell ! \sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}} \left(\prod_{i=1}^{\log_2(n)} \binom{n/2^i}{\ell_{\alpha_i}}\binom{n/2^i}{\ell_{\beta_i}}\left(\frac{2^i}{n^2}\right)^{\ell_{\alpha_i}+\ell_{\beta_i}}\right)\\
		&\leq \binom{\ell^2}{\ell} \ell ! \sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}} \left(\prod_{i=1}^{\log_2(n)} \left(\frac{n/2^i \cdot e}{\ell_{\alpha_i}}\right)^{\ell_{\alpha_i}} \left(\frac{n/2^i \cdot e}{\ell_{\beta_i}}\right)^{\ell_{\beta_i}} \left(\frac{2^i}{n^2}\right)^{\ell_{\alpha_i}+\ell_{\beta_i}}\right)\\
		&= \binom{\ell^2}{\ell} \ell ! \sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}} \left(\prod_{i=1}^{\log_2(n)} \left(\frac{1}{\ell_{\alpha_i}}\right)^{\ell_{\alpha_i}} \left(\frac{1}{\ell_{\beta_i}}\right)^{\ell_{\beta_i}} \left(\frac{e}{n}\right)^{\ell_{\alpha_i}+\ell_{\beta_i}}\right)\\
		&= \binom{\ell^2}{\ell} \ell ! \left(\frac{e}{n}\right)^{\ell} \sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}}  \left(\prod_{i=1}^{\log_2(n)} \left(\frac{1}{\ell_{\alpha_i}}\right)^{\ell_{\alpha_i}} \left(\frac{1}{\ell_{\beta_i}}\right)^{\ell_{\beta_i}} \right)\\
		&\leq \binom{\ell^2}{\ell} \ell ! \left(\frac{e}{n}\right)^{\ell} \sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}} 1
	\end{align*}

 }

 \jt{

 Using $\binom{n/2^i}{\ell_{\alpha_i}}\le (n/2^i)^{\ell_{\alpha_i}}$ and $\binom{n/2^i}{\ell_{\beta_i}}\le (n/2^i)^{\ell_{\beta_i}}$,
 we have
 \[
p_S\le \binom{\ell^2}{\ell} \ell ! n^{-\ell} \sum_{{\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}} 1.
 \]
 }
	\jc{was: Then, as the number of different value assignments for the variables $\ell_{\alpha_i}$ and $\ell_{\beta_i}$ for $1 \leq i \leq \ln(n)$ is $\binom{\ell + 2\log_2(n) -1}{2\log_2(n)-1}$ based on the standard combinatorial problem of distributing indistinguishable balls over distinguishable boxes,}
 \jt{The set of $\{({\boldsymbol \ell_{\alpha}},{\boldsymbol \ell_{\beta}}):\sum_{i=1}^{\log_2(n)} \left(\ell_{\alpha_i}+\ell_{\beta_i}\right)= \ell\}$ corresponds to the set of weak integer compositions of $\ell$ into $2\log_2 n$ parts of nonnegative integers, and thus has cardinality $\binom{\ell + 2\log_2 n -1}{2\log_2 n-1} \le \binom{\ell + 2\log_2 n }{\ell}$.}

 \jc{deleted: 
 \begin{align*}
	    p_s &\leq \binom{\ell^2}{\ell} \ell ! \left(\frac{e}{n}\right)^{\ell} \binom{\ell + 2\log_2(n)}{2\log_2(n)}
	\end{align*}
}	
	Thus, it follows that
	\begin{align*}
		\mathbb{E}[X] &\leq \sum_{\ell = 1}^{\sqrt{\ln(n)}} \mathbb{E}[\ell Z_{\ell}]\\
		&= \sum_{\ell = 1}^{\sqrt{\ln(n)}} \left(\ell \cdot \sum_{S \in \binom{[n]}{\ell}} p_S \right)\\
		&\leq \sum_{\ell = 1}^{\sqrt{\ln(n)}} \ell \binom{n}{\ell} \binom{\ell^2}{\ell} \ell ! \jt{n}^{-\ell} \binom{\ell + 2\log_2(n)}{\jt{\ell}}.
%		&\leq \sum_{\ell = 1}^{\sqrt{\ln(n)}} \ell \frac{n^{\ell}}{\ell !} \binom{\ell^2}{\ell} \ell ! \left(\frac{e}{n}\right)^{\ell} \binom{\ell + 2\log_2(n)}{2\log_2(n)}\\	
%		&= \sum_{\ell = 1}^{\sqrt{\ln(n)}} \ell \binom{\ell^2}{\ell} e^{\ell} \binom{\ell + 2\log_2(n)}{2\log_2(n)}\\				
%		&\leq \sum_{\ell = 1}^{\sqrt{\ln(n)}} \ell \left(\frac{e \cdot \ell^2}{\ell}\right)^{\ell} e^{\ell} \binom{\ell + 2\log_2(n)}{2\log_2(n)}\\	
%		&= \sum_{\ell = 1}^{\sqrt{\ln(n)}} \ell \cdot e^{2\ell} \ell^{\ell} \binom{\ell + 2\log_2(n)}{2\log_2(n)}\\	
%		&\leq \sqrt{\ln(n)}\cdot \sqrt{\ln(n)} \cdot e^{2\sqrt{\ln(n)}} \sqrt{\ln(n)}^{\sqrt{\ln(n)}} \binom{\sqrt{\ln(n)} + 2\log_2(n)}{2\log_2(n)}\\  
%		&= \ln(n) \cdot e^{2\sqrt{\ln(n)}} \sqrt{\ln(n)}^{\sqrt{\ln(n)}}  \binom{\sqrt{\ln(n)} + 2\log_2(n)}{\sqrt{\ln(n)}}\\
%		&\leq \ln(n) \cdot e^{2\sqrt{\ln(n)}} \sqrt{\ln(n)}^{\sqrt{\ln(n)}} \cdot \left(\frac{e\left(\sqrt{\ln(n)} + 2\log_2(n)\right)}{\sqrt{\ln(n)}}\right)^{\sqrt{\ln(n)}}\\
%		&= \ln(n) \cdot e^{3\sqrt{\ln(n)}} \cdot \left(\sqrt{\ln(n)} + 2\log_2(n)\right)^{\sqrt{\ln(n)}}.
	\end{align*}

\jt{Using $\binom{n}{\ell}\le n^{\ell}/\ell!$, $\binom{\ell^2}{\ell}\le (e\ell)^{\ell}$ and $\binom{\ell + 2\log_2(n)}{\ell} \le (e(\ell+\log_2 n)/\ell)^{\ell} \le (10\log_2 n/\ell)^{\ell}  $ (as $\ell\le \sqrt{\ln n}$), we obtain
\[
\ex{X}\le \sum_{\ell = 1}^{\sqrt{\ln(n)}}  \ell (10 e \log_2 n)^{\ell} = \exp\left( \sqrt{\ln n}\ln\log_2 n+O(\sqrt{\ln n})\right)=o(n),
\]

}

\jc{Can you do a global search and change all $\log_2(n)$ to $\log_2 n$? Similarly, $\ln(n)$ should change to $\ln n$.}

 \jc{ deleted: 
	Then, 
	\begin{align*}
		\lim\limits_{n \to \infty} \frac{\mathbb{E}[X]}{n} &\leq \lim\limits_{n \to \infty} \frac{\ln(n) \cdot e^{3\sqrt{\ln(n)}} \cdot \left(\sqrt{\ln(n)} + 2\log_2(n)\right)^{\sqrt{\ln(n)}}}{n}\\
		&\leq \lim\limits_{n \to \infty} \frac{\ln(n) \cdot e^{3\sqrt{\ln(n)}} \cdot \left(3\log_2(n)\right)^{\sqrt{\ln(n)}}}{n}\\
		&= \lim\limits_{n \to \infty} \frac{\exp{\left(\ln(\ln(n)) + 3\sqrt{\ln(n)} + \ln\left( \left(3\log_2(n)\right)^{\sqrt{\ln(n)}}\right) \right)}}{n}\\
		&= \lim\limits_{n \to \infty} \frac{\exp{\left(\ln(\ln(n)) + 3\sqrt{\ln(n)} + \sqrt{\ln(n)} \cdot \ln\left( 3\log_2(n)\right) \right)}}{n}\\
		&\leq \lim\limits_{n \to \infty} \frac{\exp{\left(\sqrt{\ln(n)} \cdot \ln\left( 5\log_2(n)\right) \right)}}{n}\\
		&= \lim\limits_{n \to \infty} \frac{(5 \log_2(n))^{\sqrt{\ln(n)}}}{n}\\
		&= 0,
	\end{align*}
 }
	as desired.
\end{proof}
\begin{corollary}
    \label{cor:2-connectedness_number_of_components}
    Let $G$ be the semi-random graph resulting from the $2$-min process. Then, a.a.s., $G$ contains $o(n)$ maximal $2$-connected induced subgraphs.
\end{corollary}
\begin{proof}
    By Proposition~\ref{prop:2-connectedness_small_blocks} there are $o(n)$ maximal $2$-connected induced subgraphs of order at most $\sqrt{\ln(n)}$. 
    \jt{Let $\cal{B}$ denote the set of blocks of $G$. Consider the set ${\cal T}:=\{(v,B): v\in B, B\in {\cal B}\}$. Using the block-cut tree structure in Definition~\ref{def:block-cut_tree}, $|{\cal T}|= n+|{\cal B}| - 1$. Moreover, ${\cal T}_B:=\{(v',B')\in T: B'=B\}$ partitions ${\cal T}$. Let $B_{1},\ldots, B_{\ell}$ be the set of blocks of size at least $\sqrt{\ln n}$. Then, $\sum_{1\le i\le \ell} |{\cal T}_{B_i}| \le |{\cal T}| = n+\ell+o(n)$, as we have shown that the number of blocks of size smaller than $\sqrt{\ln n}$  is $o(n)$. However, $|{\cal T}_{B_i}|\ge \sqrt{\ln n}$ for every $i$, and thus it follows then that $\ell \sqrt{\ln n} \le n+\ell +o(n)$, which implies that $\ell=o(n)$. The assertion of the corollary follows. }
    
    \jc{was: Moreover, by the construction of the block-cut graph (see Definition~\ref{def:block-cut_tree}) we note that the number of vertices shared by multiple maximal $2$-connected induced subgraphs is bounded by the number of maximal $2$-connected induced subgraphs. Thus, the number of maximal $2$-connected induced subgraphs of order at least $\sqrt{\ln(n)}$ is at most $n / (\sqrt{\ln(n)}-1) = o(n)$. Hence, there are $o(n)$ maximal $2$-connected induced subgraphs, as desired.}
\end{proof}

\jt{Let $G_1$ be the graph obtained after the first phase, i.e.\ the graph resulting from the 2-min process.} In the second phase, we \jt{add semi-random edges to make $G_1$ connected.} The following proposition shows that we can achieve this \jt{with $o(n)$ additional semi-random edges}. 
\begin{proposition}
    \label{prop:2-connectedness_connect}
    A.a.s.\ $G_1$ \jt{can be made connected by adding} $o(n)$ \jt{semi-random edges}.
\end{proposition}
\begin{proof}
    By Corollary~\ref{cor:2-connectedness_number_of_components}, $G_1$ contains $o(n)$ maximal $2$-connected induced subgraphs. We claim that each vertex not contained in a $2$-connected induced subgraph is contained in a component that contains a $2$-connected induced subgraph. Suppose not. \jc{you can keep this for your thesis. For the paper I would delete this: Then let $C$ be a component of graph $G_1$ not containing $2$-connected induced subgraph. Hence, component $C$ is acyclic, and thus a tree. However, each leaf of the tree has degree $1$, contradicting the result of the $2$-min process.} \jt{Then $G_1$ must contain a tree component, contradicting with the fact that the minimum degree of $G_1$ is at least two.} Hence the number of components of graph $G_1$ is bounded from above by the number of maximal $2$-connected induced subgraphs, and therefore is $o(n)$.
    
    \jc{slightly reworded, you may keep your version for your thesis: We moreover note that each round, in a disconnected graph, we can decrease the number of connected components by 1. Namely, for vertex $u$ being chosen u.a.r., we select vertex $v$ u.a.r. in a different connected component than vertex $u$. Hence, a.a.s., in $o(n)$ additional rounds, we can ensure graph $G$ to be connected, as desired.}
    \jt{Note that each semi-random edge can decrease the number of components by 1, by choosing $v_t$ that lies in a different component as $u_t$ before the addition of $u_tv_t$. Hence, $G_1$ can be made connected by $o(n)$ semi-random edges.}
\end{proof}



\jt{Let $G_2$ be the graph obtained after phase 2.} In the third phase, we \jt{make $G_2$} $2$-connected \jt{by adding $o(n)$ semi-random edges}. %The following proposition shows that we can also make this phase efficient.
\begin{proposition}
    \label{prop:2--edge-connectedness}
    %Let $G$ be the semi-random graph resulting from the $2$-min process. Then, a.a.s. it takes $o(n)$ additional rounds to ensure that graph $G$ is $2$-edge-connected.\
    \jt{$G_2$ can be made $2$-connected by the addition of $o(n)$ semi-random edges.}
\end{proposition}
\begin{proof}
    \jc{Deleted: By Proposition~\ref{prop:2-connectedness_connect}, a.a.s. it takes $o(n)$ to ensure that graph $G$ is connected. Hence, we may assume that graph $G$ is connected. Then} Let \jt{$\mathcal{B}$ be a block decomposition of $G_2$ and} $T_{\mathcal{B}}$ be a reduced block tree of $G_2$. By Proposition~\ref{prop:reduced_block_tree_leaves}, each leaf in $T_{\mathcal{B}}$ is a $2$-connected block. Thus, by Corollary~\ref{cor:2-connectedness_number_of_components}, $T_{\mathcal{B}}$ a.a.s. contains $o(n)$ leaves.

%    Suppose that $e$ is a cut-edge in graph $G_2$. Then, by the definition of blocks, $e$ corresponds to a block $B_e$ of size $2$ in $\mathcal{B}$. \jt{Let ${\cal C}$ denote the set of cut-edges in $G_2$ and let $\{B_e: e\in {\cal C}\}$ be the set of blocks corresponding to $e\in {\cal C}$.} Thus, each such \jt{$B_e$} corresponds to an internal vertex of $T_{\mathcal{B}}$. \jt{For each $e\in {\cal C}$,} let $L_{B_e} \subseteq V(T_{\mathcal{B}})$ be the set of leaves $B'$ in $T_{\mathcal{B}}$ such that block $B$ is on the unique path between $B^*$ and leaf $B'$ in $T_{\mathcal{B}}$. We observe that adding an edge \jt{to $G_2$} between \jt{a vertex in} $B^*$ and \jt{a vertex in} $B'$ for each leaf $B' \in L_B$ suffices to ensure that edge $e$ is no longer a cut-edge in $G_2$. \jc{I deleted the following. This is exactly where I ran into trouble before. } \jc{Deleted: Because this holds for all cut-edges in $G_2$, it suffices to add edges between $B^*$ and all leaves in $T_{\mathcal{B}}$ in order to ensure $G_2$ is $2$-edge-connected.} 
    

    
    First consider the case \jc{was: that block decomposition $\mathcal{B}(G)$} \jt{${\cal B}$} contains a block $B^*$ such that $|B^*| \geq n / 4$. We consider the following strategy. Take an arbitrary enumeration $B_1,\ldots, B_h$ of all leaf blocks of $T_{\mathcal{B}}$. For each $1\le j\le h$, we will add a semi-random edge between $B^*$ and $B_j$ in increasing order of $j$, \jt{in a way that all cut vertices of $G_2$ in $\cup_{B\in P_j} B$ are no longer cut vertices after the addition of the edge, where $P_j=B_jB'_1B'_2\ldots B'_{\ell}B^*$ denotes the unique path from $B_j$ to $B^*$ in $T_{\mathcal{B}}$.} Suppose these semi-random edges have already been added between $B^*$ and $B_i$ for all $i<j$.  Moreover, let $x$ be the unique vertex in $B_j \cap B'_1$, and $y$ the unique vertex in $B'_{\ell} \cap B^*$. Note that possibly $x = y$. Then, in each subsequent round $t$, if the square (i.e.\ the first vertex) $u_t$ is contained in  $B^*\setminus \{y\}$, we let $v_t$, the circle, be an arbitrary vertex in $B_j\setminus \{x\}$. We note that by the definitions of $x$ and $y$, $u_tv_t$ cannot be an edge in $G_2$. If instead square $u_t$ is not contained in $B^* \setminus \{y\}$, we consider the round a failure.
    
    We claim that \jt{after the addition of the $h$ semi-random edges as described above,} the resulting graph $G_3$ no longer contains cut-vertices. Suppose for the sake of contradiction that $G_3$ does contain a cut-vertex $v$. \jt{Then $v$ must be a cut-vertex in $G_2$.} Let $C_1, C_2$ be two components of $G_2 - v$ such that $B^* \setminus \{v\}$ is contained in $C_1$. We then observe that $C_2$ has to contain \jt{$B_i \setminus \{v\}$, where $B_i$ was a leaf in $T_{{\cal B}}$}. However, by the definition of $x$ and $y$, the semi-random edge \jt{$e$} added between $B^*$ and $B_i$ does not have $v$ as an endpoint. Hence, $C_1$ and $C_2$ are connected by \jt{$e$}, a contradiction.
    
    Note that in each round, the probability of the first vertex landing in $B^*\setminus \{y\}$ is $(|B^*|-1)/n \geq 1/4-o(1)$, and as a.a.s.\ $T_{\mathcal{B}}$ contains $o(n)$ leaves, the number of rounds required to add semi-random edges between $B^*$ and all $B_1,\ldots, B_h$ is $o(n)$ in expectation. Standard concentration inequalities such as Chernoff bounds immediately imply that a.a.s.\ it takes $o(n)$ rounds to extend $G_2$ to a 2-connected graph. 
    
    Hence we may assume that each block $B$ in $\mathcal{B}$ is of size strictly smaller than $n/4$. We use a different strategy in this case. Instead of adding edges from leaves to a single block, we will consider balancing the tree into two subforests. We will then add edges between the leaves in one forest and vertices in the other forest, and vice versa.
    
    Let vertex ${B^*} \in V(T_{\mathcal{B}})$, coloring $\phi : V(T_{\mathcal{B}}) \setminus \{B^*\} \to \{\text{red$,$ blue}\}$, and sets $S_{\text{red}}$ and $S_{\text{blue}}$ be as given by Proposition~\ref{prop:reduced_block_tree_balanced}. For each $v \in B^*$ let $T_{\mathcal{B}, v}$ denote the components of $T_{\mathcal{B}} - v$ that contain a block containing $v$. Thus, $T_{\mathcal{B}, v}$ denotes the blocks $B$ where $v$ is the last cut-vertex on the path from $B$ to $B^*$ in $T_{\mathcal{B}}$. We refer to $T_{\mathcal{B}, v}$ as the branch rooted at $v$. Moreover, let $S_{\mathcal{B}, v}$ denote $\bigcup_{B \in V(T_{\mathcal{B}, v})} B \setminus B^*$. That is, $S_{\mathcal{B}, v}$ is the set of all vertices contained in blocks in $T_{\mathcal{B}, v}$ except for vertex $v$ itself. If $|S_{\mathcal{B}, v}| \leq n/8$, we say branch $T_{\mathcal{B}, v}$ is small. Otherwise we say $T_{\mathcal{B}, v}$ is big. Finally, for all leave blocks $B$, let $v_{B}$ denote the vertex that block $B$ has in common with the next block on the path from $B$ to $B^*$ in $T_{\mathcal{B}}$
    
    We first consider the leaves of $T_{\mathcal{B}}$ contained in small branches. Take two arbitrary enumerations $B_1, B_2, \ldots, B_{h_1}$ and $R_1, R_2, \ldots, R_{h_2}$ of all blue and red leaf blocks of $T_{\mathcal{B}}$ contained in small branches respectively. We will iteratively add edges between $S_{\text{red}}$ and $B_j$ in increasing order of $j$, and analogously between $S_{\text{blue}}$ and $R_j$. Suppose that semi-random edges have already been added between $S_{\text{red}}$ and $B_i$ for all $i < j$. Let $T_{\mathcal{B}, v}$ be the branch containing leaf $B_j$. Then, if square $u_t$ lands in $S_{\text{red}} \setminus S_{\mathcal{B}, v}$, we choose circle $v_t$ to be an arbitrary vertex in $B_j \setminus \{v_{B_j}\}$. Because $|B_j| \geq 2$, such a choice for $v_t$ always exists. Because $u_t$ and $v_t$ are in different branches, and as $u_t, v_t \not \in B^*$, it follows that edge $u_tv_t$ cannot be contained in $G_2$.
    
    Analogously, for $R_i$ the red leaf in a small branch $T_{\mathcal{B}, v}$ with the lowest index that has not previously received a circle, if square $u_t$ is contained in $S_{\text{blue}} \setminus S_{\mathcal{B}, v}$, we choose $v_t$ in $R_i \setminus \{v_{R_i}\}$. Finally, if square $u_t$ is contained in $B^*$, or in same branch as the considered leaf, we consider the round a failure.
    
    Then, as tree $T_{\mathcal{B}}$ has $o(n)$ leaves, there are $o(n)$ blue and $o(n)$ red leaves. Moreover, by Proposition~\ref{prop:reduced_block_tree_balanced} $|S_{\text{blue}}| \leq |S_{\text{red}}| \leq 3|S_{\text{blue}}|$, and $|S_{\text{red}}| + |S_{\text{red}}| \geq 3n/4$. Thus, the probability that a vertex from $S_{\text{red}} \setminus S_{\mathcal{B}, v}$ is chosen u.a.r. where $T_{\mathcal{B}, v}$ a small branch, is at least $3n/8 - n/8 = n/4$. Similarly, the probability that a vertex from $S_{\text{blue}} \setminus S_{\mathcal{B}, v}$ is chosen u.a.r. where $T_{\mathcal{B}, v}$ a small branch, is at least $3n/16 - n/8 = n/16$. Hence, the expected number of rounds needed to add edges to all leaf blocks in small branches is $o(n)$
    
    Next, we consider the leaf blocks in big branches. We first note that there are at most $8$ big branches. We use a similar strategy as for the small branches, but drop the requirement that $u_t$ and $v_t$ must be in distinct branches. Again take two arbitrary enumerations $B_1, B_2, \ldots, B_{h_3}$ and $R_1, R_2, \ldots, R_{h_4}$ of all blue and red leaf blocks of $T_{\mathcal{B}}$ contained in big branches respectively. Suppose that semi-random edges have already been added between $S_{\text{red}}$ and $B_i$ for all $i < j$. Then, if square $u_t$ lands in $S_{\text{red}}$, we choose circle $v_t$ to be an arbitrary vertex in $B_j \setminus \{v_{B_j}\}$. Because $|B_j| \geq 2$, such a choice for $v_t$ always exists. Because $u_t$ and $v_t$ are in different colour classes, and as $u_t, v_t \not \in B^*$, it follows that edge $u_tv_t$ cannot be contained in $G_2$. If $u_t$ lands in $S_{\text{blue}}$, we analogously choose $v_t$ in the considered red leaf block. If instead $u_t$ lands in $B^*$, we consider the round a failure. 
    
    Because the probability that a vertex from $S_{\text{red}}$ is chosen u.a.r. is at least $3n/8$, and the probability that a vertex from $S_{\text{blue}}$ is chosen u.a.r. is at least $3n/16$, it also takes $o(n)$ rounds in expectation to add edges to all leaf blocks in big branches. 
    
    After all leaves in both small and big branches have received an edge, there exist two internally vertex-disjoint paths from each leaf block $B$ to $B^*$. Namely, as all of the edges we added have one red and one blue endpoint, each blue leaf has a path which only contains blue vertices and a vertex in $B^*$, and a path that starts with the added edge, and then only contains red vertices and one vertex in $B^*$. Analogously, there exist two such paths from each red leaf. As these two paths do not share their endpoint in leaf $B$, we note that all
    
    Moreover, for leaves in small branches, the two paths have distinct endpoints in $B^*$. As a result, 
    
    
    We again claim that once edges have been added to all leaves, the resulting graph $G_3$ is $2$-connected. Suppose for the sake of contradiction that $G_3$ contains a cut-vertex $v$. Let $C_1, C_2$ be two components of $G_2 - v$ such that $B^* \setminus \{v\}$ is contained in $C_1$. First consider the case that $v \in B^*$. Let  
    
    Then, as tree $T_{\mathcal{B}}$ has $o(n)$ leaves, there are $o(n)$ blue and $o(n)$ red leaves. Moreover, by Proposition~\ref{prop:reduced_block_tree_balanced} $|S_{\text{blue}}| \leq |S_{\text{red}}| \leq 3|S_{\text{blue}}|$, and $|S_{\text{red}}| + |S_{\text{red}}| \geq 3n/4$. Thus, the probability that a vertex from $S_{\text{red}}$ is chosen u.a.r. is at least $3n/8$, and the probability that a vertex from $S_{\text{blue}}$ is chosen u.a.r. is at least $3n/16$. Hence, we conclude that the expected number of rounds to $G_2$ becomes $2$-connected is $o(n)$. Again concentration inequalities then imply that we obtain a $2$-connected graph a.a.s.\ in $o(n)$ rounds.
\end{proof}


In the fourth phase, we want to ensure that a large part of the graph, formed by the large blocks in graph $G$, becomes $2$-connected. In the following proposition we find that this can be done efficiently.
\begin{proposition}
	\label{prop:2-connectedness_connect_large}
	Let $G$ be the semi-random graph resulting from the $2$-min process, and let $\mathcal{B}^* \subseteq \mathcal{P}(V(G))$ be the set of the vertex sets of the $2$-connected blocks of order at least $\sqrt{\ln(n)}$ in graph $G$. Then, a.a.s., we can construct a graph $G'$ in which the vertex set $\cup_{B \in \mathcal{B}^*} B$ induces a $2$-connected graph in $O(n/(\sqrt{\ln(n)}-1))$ additional rounds.
\end{proposition}
\begin{proof}
	We will construct a $2$-connected subgraph from all blocks in set $\mathcal{B}^*$. Let $B_0 \in \mathcal{B}^*$ be an arbitrary block, and color this block red. We color the remainder of the blocks in set $\mathcal{B}^*$ blue. Let $R$ be the vertex set of the $2$-connected red subgraph constructed thus far, and hence initially $R = B_0$. Every round, we then add an edge with one red and one blue endpoint. Let $B \in \mathcal{B}^*$ be the block containing the blue endpoint. If the addition of the edge results in the subgraph induced by vertex set $R \cup B^*$ to be $2$-connected, we color block $B$ red, and update set $R$ to include the vertices in block $B$. We thus note that if $B \subseteq R$ for all $B \in \mathcal{B}^*$, the vertex set $R$ induces a $2$-connected subgraph containing all the blocks in set $\mathcal{B}^*$. 
	
	We observe that if for a blue block $B \in \mathcal{B}^*$ graph $G$ we add two vertex-disjoint red-blue edges with the blue endpoint in block $B$, block $B$ is $2$-connected with the red vertices, and therefore we color block $B$ red. Hence, it suffices to add at most two red-blue vertex-disjoint edges for each block in set $\mathcal{B}^*$. Every round, we attempt to place such a red-blue edge that is vertex-disjoint with previously placed edges with endpoints in the same blue block. If that is not possible, we consider the round a failure. 
	
	First consider the case that the first vertex in a round, chosen uniformly at random, is a blue vertex. Let $B \in \mathcal{B}^*$ be the blue block containing said vertex. As there exists at most one vertex-disjoint edge between sets $R$ and $B$, there is at most one vertex in set $B$ that would lead to a failure round. As set $B$, by the definition of set $\mathcal{B}^*$ is of order at least $\sqrt{\ln(n)}$, the probability that the round is a failure if the first vertex is blue, is at most $1/\sqrt{\ln(n)}$.
	
	Next, consider the case that the first vertex in a round is a red vertex. We note that this round is a failure if and only if this uniformly at random chosen vertex is adjacent to vertices in each blue block. Moreover, it is only a failure round if it is the only such vertex. Then, as $|R| \geq |B_0| \geq \sqrt{\ln(n)}$, also in this case the probability that the round is a failure is at most $1/\sqrt{\ln(n)}$. 
	
	Finally, if the first vertex chosen in a round is neither a blue nor a red vertex, that is the vertex lies in a $2$-connected block of order at most $\sqrt{\ln(n)}$, we also consider the round a failure. However, as by Proposition~\ref{prop:2-connectedness_small_blocks} there are $o(n)$ such blocks, containing in total $o(n)$ vertices, the probability of choosing one such vertex uniformly at random is also $o(n)$. Hence, for $n \to \infty$, a.a.s. the number of failure rounds as a result of hitting such vertices is $O(1)$. Therefore, for the remainder of the proof, we may assume that this case does not occur.
	
	Thus, in both the case that the first vertex is blue, as in the case that the first vertex is red, the probability of a round being a failure is at most $1/\sqrt{\ln(n)}$. Moreover, we note that by the structure of the traditional block tree, the number of cut-vertices in a graph is strictly smaller than the number of blocks in a graph. Hence, as there is thus less than 1 cut-vertex per block on average, there are at most $n / (\sqrt{\ln(n)}-1)$ blue blocks. Therefore, we need at most $2n / (\sqrt{\ln(n)}-1)$ successful rounds. We claim that a.a.s., $3n/(\sqrt{\ln(n)}-1)$ rounds suffice.
	
	Let $X$ be a binomial random variable with $3n/(\sqrt{\ln{(n)} - 1}$ trials and success probability $1/\sqrt{\ln{n}}$ and coupled with the number of failure rounds in $3n/(\sqrt{\ln{(n)}} - 1)$ rounds to provide an upper bound on said number. Then, using the Chernoff-Hoeffding bound, and as $\mathbb{E}[X] \leq \frac{1}{\sqrt{\ln{(n)}}} \cdot \frac{3n}{\sqrt{\ln(n)} -1}$,
	\begin{align*}
		\mathbb{P}\left(X > \frac{\sqrt{\ln{(n)}}}{3} \cdot \mathbb{E}[X]\right) & \leq 2^{- \frac{\sqrt{\ln{(n)}}}{3} \cdot \mathbb{E}[X]}\\
		&= 2^{- \frac{n}{\sqrt{\ln(n)}-1}}\\
		&= o(1).
	\end{align*}
	Thus, a.a.s., $X \leq n/(\sqrt{\ln(n)}-1)$. Therefore, as the number of successful rounds is $\frac{3n}{\sqrt{\ln(n)}-1} - X$, a.a.s., at least $\frac{2n}{\sqrt{\ln(n)}-1}$ of the additional rounds are successful, as desired.
\end{proof}

Finally, we have a fifth cleanup phase where we absorb the smaller blocks disregarded in the previous phase, ensuring that the entire graph becomes $2$-connected.
\begin{proposition}
	\label{prop:2-connectedness_connect_small}
	Let $G$ be the semi-random graph resulting from the $2$-min process where all $2$-connected blocks of order at least $\sqrt{\ln(n)}$ have subsequently been joined into a single $2$-connected block. Then, a.a.s., we can obtain a $2$-connected graph in $o(n)$ additional rounds.
\end{proposition}
\begin{proof}
	Let the large $2$-connected block constructed by joining the $2$-connected blocks of order at least $\sqrt{\ln(n)}$ in graph $G$ be colored red, and let all the remaining $2$-connected blocks be colored blue. Then, by Proposition~\ref{prop:2-connectedness_small_blocks} there are $o(n)$ blue vertices.
	
	Then, in each round we will add an edge with one red endpoint, and one blue endpoint. We observe that if we add two vertex-disjoint red-blue edges with endpoints in the same blue $2$-connected block, this block will form a $2$-connected subgraph with the red vertices, and hence will also be colored red. We consider each round where a blue vertex is chosen uniformly at random a failure, and similarly if a red vertex is chosen that is already connected to all remaining blue blocks. 
	
	As there are $o(n)$ blue vertices, and as there is at most one red vertex that leads to a failure round if picked uniformly at random, the probability of a round being a failure is $o(n)$. Hence, a.a.s. in $m$ additional rounds, $\Theta(m)$ of the rounds will be successful. 
	
	Thus, because by Proposition~\ref{prop:2-connectedness_small_blocks} there are $o(n)$ blue $2$-connected blocks, and as it suffices to have two successful rounds for each blue $2$-connected block, the proposition follows.
\end{proof}


Combining the analysis of these individual phases then results in the following lemma.

\begin{lemma}
    \label{lem:2-connectedness_upper_bound}
    $\tau_{\mathcal{C}_2} \leq \ln(2) + \ln(\ln(2)+1)) + o(1)$.
\end{lemma}
\begin{proof}
    	The lemma directly follows from Propositions~\ref{prop:2-connectedness_small_blocks}, \ref{prop:2-connectedness_connect_large} and~\ref{prop:2-connectedness_connect_small}, and that the $2$-min process requires $(\ln(2) + \ln(\ln(2)+1)) + o(1))n$ rounds.
\end{proof}

\subsection{Pre-positional model}
In this section, we consider $k$-connectedness in the pre-positional model. By Lemma~\ref{lem:relation_pre_post_positional}, $\tau_{\mathcal{C}_k} \leq \tau_{\mathcal{C}_k}'$ for all $k \geq 1$. The lower bounds for $\tau_{\mathcal{C}_k}$ thus apply to $\tau_{\mathcal{C}_k}'$ as well.

We observe that the case for $k=1$ is not as simple in the pre-positional model as in the post-positional model. Namely, there is no strategy to guarantee that $u_t$ and $v_t$ lie in different connected components (disregarding isolated vertices). 

\begin{lemma}
\label{lem:pre-positional_1-connectedness}
    $\tau_{\mathcal{C}_1}' = (1 + o(1))n$.
\end{lemma}
\begin{proof}
    We first observe that as $\tau_{\mathcal{C}_1} = n-1 = (1+o(1)n)$, we find the lower bound $\tau_{\mathcal{C}_1}' \geq (1 + o(1))n$.
    
    For the upper bound, we consider a strategy $\mathcal{S}$ which chooses $u_t$ u.a.r. from all vertices contained in any connected component of minimum order. If $v_t$ lands in a different connected component, we add edge $u_tv_t$. Otherwise we consider the round a failure round. Each successfully added edge then decreases the number of connected components in the graph by $1$. We analyze the process with this strategy in a number of phases. 
    
    Let phase $i$ be defined as the rounds in which the number of connected components in the graph decreases from $\frac{n}{2^{i-1}}$ to $\frac{n}{2^i}$. We note that phase $i$ consists of $\frac{n}{2^{i-1}} - \frac{n}{2^i} = \frac{n}{2^i}$ non-failure rounds, and a number of failure rounds. Let $T_i$ be the total number of rounds in phase $i$, and let $f_i$ be the number of failure rounds in phase $i$. Thus, $T_i = \frac{n}{2^{i}} + f_i$.
    
    We then observe that the smallest connected component in any round in phase $i$ contains at most $2^i$ vertices. The probability that a round is a failure round is thus at most $2^i /n$. Suppose that $T_i \leq \alpha\cdot  \frac{n}{2^i}$ for some fixed $\alpha > 1$. Then 
    \[\mathbb{E}[f_i] \leq \alpha\cdot \frac{n}{2^i} \cdot \frac{2^i}{n} = \alpha = O(1). \]
    Moreover, by Markov's inequality, it then follows that a.a.s. $f_i = O(1)$. Thus, a.a.s. $T_i = \frac{n}{2^{i}} + O(1)$.
    
    The total number of rounds needed to ensure the graph is connected is then
    \[\sum_{i > 0}T_i = \sum_{i = 1}^{\log_2(n)} \left( \frac{n}{2^{i}} + O(1)\right) \leq n + O(\log_2(n)) = (1 + o(1))n. \]
    Therefore, $\tau_{\mathcal{C}_1}' \leq (1 + o(1))n$, as desired.
\end{proof}
Thus, asymptotically, $\tau_{\mathcal{C}_1}' = \tau_{\mathcal{C}_1}$.

To prove the tight upper bound in the post-positional model for $k \geq 3$, Ben-Eliezer et~al.~\cite{Ben-Eliezer2020Semi-randomProcess} introduce a strategy $\mathcal{S}_{\text{min}}^*$. This strategy chooses vertex $v_t$ u.a.r. from all vertices of $V(G_{t-1}) \setminus \{u_t\}$ that have the smallest number of distinct neighbours. Note that this process generates a multi-graph, and is therefore not quite equivalent to the min-degree process. They then analyze the graph resulting from this strategy in the post-positional process to show the tight upper bounds. 

We note that strategy $\mathcal{S}_{\text{min}}^*$ can be modelled in the pre-positional process by the following strategy: we choose $u_t$ u.a.r. from all vertices that have the smallest number of distinct neighbours, and consider the round a failure if $u_t = v_t$. The probability of any given round being a failure round is thus $1/n$. Hence, the number of additional rounds needed to cover the additional failure rounds is a.a.s. $o(n)$. The tight upper bounds for $\tau_{\mathcal{C}_k}$ for $k \geq 3$ thus are also tight upper bounds for $\tau_{\mathcal{C}_k}'$. Hence, Lemma~\ref{lem:pre-positional_k-connectedness} follows.

\begin{lemma}
\label{lem:pre-positional_k-connectedness}
    $\tau_{\mathcal{C}_k}' = \tau_{\mathcal{C}_k}$ for all $k \geq 3$.
\end{lemma}

The remaining open case in the pre-positional process is thus $k = 2$. We will consider the proof we have given for the tight upper bound for the post-positional case.

As discussed in Section~\ref{subsection:min-degree_process}, the pre-positional process can be used to model the min-degree process in a similar fashion to the post-positional model. Hence, it suffices to consider the phases of the proof where we define and use different strategies.

We first note that connecting the graph in the second phase is not achievable with the same strategy as in the proof of Proposition~\ref{prop:2-connectedness_connect}. Instead we use the same strategy defined in the proof of Lemma~\ref{lem:pre-positional_1-connectedness}. By analogous analysis, it then follows that Proposition~\ref{prop:2-connectedness_connect} also holds in the pre-positional process.

Next, we consider the third phase, in which we aim to ensure that the graph is $2$-edge-connected. In the proof of Proposition~\ref{prop:2-edge-connectedness}, there are two cases to examine. \textcolor{blue}{TODO - rewrite} Hence, taking into account the other bounds on the number of failure rounds considered in the proof of Proposition~\ref{prop:2-edge-connectedness}, we conclude that Proposition~\ref{prop:2-edge-connectedness} also holds for the pre-positional process.

We use a similar strategy in the fourth phase, where we ensure that the large part of the graph, formed by the large blocks, becomes $2$-connected. We again use the strategy of choosing $u_t$ to be a vertex of the least prevalent colour. By analysis analogous to that used in the proof of Proposition~\ref{prop:2-connectedness_connect_large}, it then follows that also Proposition~\ref{prop:2-connectedness_connect_large} holds for the pre-positional process. The same strategy, and similar reasoning shows that also Proposition~\ref{prop:2-connectedness_connect_small} holds for the pre-positional process.

As thus all phases of the upper bound algorithm for the post-positional process can be modelled by similar strategies in the pre-positional process, with asymptotically equal results, Lemma~\ref{lem:pre-positional_2-connectedness} follows.

\begin{lemma}
\label{lem:pre-positional_2-connectedness}
    $\tau_{\mathcal{C}_2}' = \tau_{\mathcal{C}_2}$.
\end{lemma} 

Theorem~\ref{thm:equality_models_k-connectedness} then directly follows from Lemmas~\ref{lem:pre-positional_1-connectedness},~\ref{lem:pre-positional_k-connectedness}, and~\ref{lem:pre-positional_2-connectedness}. 


==> Main_sections/minors.tex <==
\section{Minors}
\label{subsection:minors}

\begin{definition}
    A \emph{$1$-subdivision} of a graph $H$ is the graph obtained by subdividing each edge in $E(H)$ exactly once.
\end{definition}

\begin{theorem}
\label{thm:1-subdivision}
    Let $H$ be a fixed graph, and let $f: \mathbb{N} \to \mathbb{N}$ be a function such that $\lim_{n \to \infty}f(n) = \infty$. Then there exist strategies in both the pre- and post-positional processes such that the resulting graph $G$ contains a $1$-subdivision of $H$ in a.a.s.\ $f(n)\cdot n^{1/2}$ rounds.
\end{theorem}
\begin{proof}
    We proceed by induction on $|V(H)|$. Note that the theorem holds for $H$ being a single vertex. Suppose that the theorem holds for all graphs $H^*$ with $|V(H^*)| < |V(H)|$.

    \textcolor{cyan}{To complete.}
\end{proof}

We note that $1$-subdivisions are minors of their respective base graphs, the strategies given by Theorem~\ref{thm:1-subdivision} suffice to construct minors, as stated in the following corollary.
\begin{corollary}
    For $H$ a fixed graph and $f: \mathbb{N} \to \mathbb{N}$ a function such that $\lim_{n\to\infty}f(n) = \infty$, there exist strategies in both the pre- and post-positional processes such that the resulting graph $G$ contains an $H$-minor of $H$ in a.a.s.\ $f(n)\cdot n^{1/2}$ rounds.
\end{corollary}

